LLM-PQA: LLM-enhanced Prediction Query Answering

The advent of Large Language Models (LLMs) provides an opportunity to change the way queries are processed, moving beyond the constraints of conventional SQL-based database systems. However, using an LLM to answer a prediction query is still challenging, since an external ML model has to be employed and inference has to be performed in order to provide an answer. This paper introduces LLM-PQA, a novel tool that addresses prediction queries formulated in natural language. LLM-PQA is the first to combine the capabilities of LLMs and retrieval-augmented mechanism for the needs of prediction queries by integrating data lakes and model zoos. This integration provides users with access to a vast spectrum of heterogeneous data and diverse ML models, facilitating dynamic prediction query answering. In addition, LLM-PQA can dynamically train models on demand, based on specific query requirements, ensuring reliable and relevant results even when no pre-trained model in a model zoo, available for the task.

==> sections/implementation.tex <==
\section{Demonstration}


\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{figures/screenshot.png}
  \caption{Interface: query answering with matched model}
  \label{fig:UI}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{figures/screenshot_2.png}
  \caption{Interface: model training when no model is found}
  \label{fig:UI-train}
\end{figure}

: \ziyu{Output format need to be adjusted. Highlight the results}


In this section, we demonstrate our proposed framework for ML inference query answering, presented as in Figure~\ref{fig:UI} and Figure~\ref{fig:UI-train}.

User would interact with our framework by chatting with a chatbot. The chatbot receives user inputs and displays system responses, facilitating an intuitive and interactive query process.
As seen in Figure~\ref{fig:UI}, in the beginning, no model is identified that can answer the query.





==> sections/introduction_old.tex <==
\section{Introduction}

Machine learning (ML) is increasingly recognized as a transformative force in enhancing decision-making processes within both commercial enterprises and scientific research in various domains~\cite{}. 
They are widely applied in production scenarios, including credit-card fraud prediction, recommendation, business intelligence, etc, over tabular data such as transaction records and customer profiles.
\ziyu{Rephrase}



With this trend, many research as well as enterprises investigate integrating ML models within databases, also referred as in-database ML~\cite{park2022end,klabe2023exploration,guan2023comparison,foufoulas2023efficient,paganelli2023pushing}.
These works aim to exploit the power of advanced database systems and enable the data engine with the ML capability.
The ML models are encapsulated into fine-grained user defined functions (UDFs)~\cite{makrynioti2019declarative,guan2023comparison} or pushed down and decomposed into steps executed into the database execution engine~\cite{park2022end,klabe2023exploration,paganelli2023pushing}.
In this line of work, ML tasks is expressed using SQL-like format. Users define the needs by specifying fine-grained details, e.g., dataset, features, as well as specific model to use.
Writing such query require users to have sufficient understanding on the underneath datasets as well as the ML models, finding the suitable ones to match the task. 




% \para{Answering ML inference query}
% With the integration of ML inference, we are able to obtain new knowledge from the existing work and able to answer queries with specific tasks, which reduce the risk of hallucination and expand the capability of query answering.
% There are also abundant research on optimizing ML inference queries in database field in recent years, in particular for query large unstructured data, such as video. Representatives work include NoScope~\cite{kang2017noscope}, CORE~\cite{yang2022optimizing}. This line of work exploits the traditional query optimization technique and focus on the efficiency side by applying proxy model for early filtering. 


In this demo, we propose to address such ML queries, using natural language.
For example, given a dataset regarding insurance charges, a user may be interested to known the insurance charges for a particular case, e.g., a 19-year-old female, smoker, with BMI of 27.9.
If this data record does not exist in the database, ML inference needs to be performed to obtain the result.
This paper demonstrates a tool for answering such ML inference queries,
In particular, we allow for answering queries on diverse domains and tasks, by fully exploiting a data lake and model zoo.
This enables access to a broad spectrum of heterogeneous data and a diverse array of ML models, enhancing the system's ability to dynamically interact with various models and datasets. The concept of a data lake~\cite{hai2016constance,nargesian2019data}, involves storing a vast amount of raw data in its native format, which our system leverages to ensure that all available information can be utilized effectively during the inference process. 
Similarly, the model zoo~\cite{onnx,kaggle} component provides a large collection of pre-trained models that can be employed to address specific tasks.


To address this problem, we leverage the advanced capabilities of Large Language Models (LLMs).
%and a retrieval-augmented mechanism.
LLMs have proven to be effective in advancing the fields of language understanding and reasoning, facilitating translating natural language into executable SQL queries~\cite{fu2023catsql,zhang2024benchmarking}. 
However, answering such ML inference queries using only LLMs can be challenging.
% First, LLMs lack specialized domain knowledge and rely heavily on the information they were trained on, making them inadequate for tasks requiring up-to-date or domain-specific data. 
% They also lack direct access to real-time data and are not inherently designed to execute specific ML operations such as predictions or classifications. 
First, LLMs generally do not cope with long context~\cite{li2023long}, taking restricted number of tokens as inputs.
Given the situation that we aim to exploit multiple models and datasets, LLMs may fall short in processing the vast amount of data.
Additionally, LLMs are ill-equipped to process raw data forms like numerical data without significant preprocessing. The complexity of ML queries, which often involve multiple interconnected steps, further complicates their use, as LLMs do not manage workflows or maintain query states. 
This limitation can lead to error propagation and challenges in debugging, especially if the model misinterprets queries or data instructions.


% \asterios{At this stage, the reader does not know how the model zoo and everything fits together. You need a solid paragraph that says that models are oin zoos, datasets in datalakes and when you ask a question you do not know what to choose to answer your query. This work crawls a model zoo, as well as a data lake of datasets, makes the match-making with metadata (what dataset is used in what model in the zoo) and then chooses the appropriate model to answet the user query. This is done in the folliwng way (and you refer to the figures).}





% \para{Challenges}
% 

% \para{RAG}
% To effectively address these issues, integrating LLMs with systems like Retrieval-Augmented Generation (RAG), specialized databases, and dynamic data handling technologies is necessary, enhancing their capability to deliver accurate and contextually relevant responses.
% RAG operates by first retrieving relevant documents or data snippets from a vast corpus based on the input query. This is typically accomplished using a vector-based search where the query and documents are transformed into embeddings in a high-dimensional space, allowing for the retrieval of the most semantically related content.
% The integration of RAG further enhances this capability by ensuring that the generated responses are both contextually focused and informed by the most current data available.


% We introduce an innovative demonstration that utilizes LLMs and augmented inputs for handling the ML inference queries, markedly improving the accuracy and applicability of responses within enterprise systems.
% Innovatively, \ziyu{DEMONAME} capitalizes on the concept of a data lake and model zoo, offering users the unprecedented ability to compose queries that tap into heterogeneous data sources and leverage a diverse collection of models with varying performance capabilities. 

The core innovation of our system lies in its integration of a retrieval-augmented mechanism with a data lake and model zoo.
The datasets and models are regarded as entities and ready for retrieval to answer the query. 
By adopting the retrieval-augmented generation (RAG) mechanism, these entities are indexed as vectors and retrieved given the user inputs. 
This approach not only broadens the scope of queries that can be effectively addressed but also enhances the framework's ability to generate insights, thus overcoming some of the inherent limitations observed when only using LLMs.
This demo presents the preliminary step of addressing ML inference query in natural language, which lay the foundation for further investigation, more complex query with multiple models and tasks involved. The framework that we propose can serve as the skeleton that allows for more enhancement.

% Our demonstration redefines the scope of query answering by introducing a new type of query that extends beyond conventional data retrieval to include direct ML inference tasks. This approach allows for more flexible interactions with a broad array of models and datasets, significantly enhancing the system's adaptability to the continuously evolving landscape of enterprise queries. By enabling dynamic access to diverse computational models and datasets, our system facilitates more nuanced and actionable insights, thereby pushing the boundaries of what is achievable with current ML and data retrieval technologies.

In the following sections, we will outline the architecture and implementation of our proposed tool, demonstrating its efficacy in handling complex ML inference queries. 
We aim to showcase practical applications and the operational viability of this tool, emphasizing its potential to address different ML tasks. 
% This paper not only contributes to academic discourse but also provides a practical blueprint for future advancements in the integration of ML into data retrieval systems.




% \para{Contributions}
% \begin{itemize}
%     \item A framework for ML inference exploiting LLM and vector search.
%     \item Integrate data lake and model zoo to support more advanced queries.
% \end{itemize}
